FairSight: Visual Analytics for Fairness in Decision Making

Data-driven decision making related to individuals has become increasingly pervasive, but the issue concerning the potential discrimination has been raised by recent studies. In response, researchers have made efforts to propose and implement fairness measures and algorithms, but those efforts have not been translated to the real-world practice of data-driven decision making. As such, there is still an urgent need to create a viable tool to facilitate fair decision making. We propose FairSight, a visual analytic system to address this need; it is designed to achieve different notions of fairness in ranking decisions through identifying the required actions -- understanding, measuring, diagnosing and mitigating biases -- that together lead to fairer decision making. Through a case study and user study, we demonstrate that the proposed visual analytic and diagnostic modules in the system are effective in understanding the fairness-aware decision pipeline and obtaining more fair outcomes.

==> 04_method.tex <==
\begin{table*}
    \caption{Fair Decision Making Framework \& FairSight Methods}
    \label{tbl:framework}
    \begin{center}
    \begin{tabular}{lllll}
      \toprule
      Pipeline & Task & Data & Model & Outcome  \\
      \midrule
      
      \begin{tabular}{@{}l@{}} 
      Understand
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      \textit{Can we understand how individuals} \\
      \textit{and groups are distributed?}
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Input space
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Mapping Space
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Output space
      \end{tabular} & \\
      
      \begin{tabular}{@{}l@{}} 
      Measure  
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      \textit{Can we measure and summarize} \\ 
      \textit{biases?}
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      \end{tabular} &
      \begin{tabular}{@{}l@{}}
      \end{tabular} & \\
      
      \begin{tabular}{@{}l@{}} 
      \hspace{3mm}Instance-level
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      \textit{Is an individual not treated similarly?} \\
      \textit{Is the distortion advantaged or} \\
      \textit{disadvantaged?}
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      -
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      rNN \\
      rNN-gain
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      -
      \end{tabular} & \\
      
      \begin{tabular}{@{}l@{}} 
      \hspace{3mm}Individual \\
      \hspace{3mm}fairness
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      \textit{Are similar individuals treated} \\ 
      \textit{similarly?}
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      -
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      rNN-mean
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      -
      \end{tabular} & \\
      
      \begin{tabular}{@{}l@{}} 
      \hspace{3mm}Group \\
      \hspace{3mm}fairness
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      \textit{Are groups treated equally?}
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Group Separation \\
      (Hausdorff Distance)
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Group Skew
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      GFDCG
      \end{tabular} & \\
      
      \begin{tabular}{@{}l@{}} 
      \hspace{3mm}Utility
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      \textit{How is the model accurate?}
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      -
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      -
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Between: linear nDCG \\
      Within: Precision
      \end{tabular} & \\
      
      \begin{tabular}{@{}l@{}}
      Identify  
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      \textit{Can we identify features} \\ 
      \textit{as a potential source of bias?}
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Feature Correlation
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Feature distortion
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Feature perturbation
      \end{tabular} & \\

      \begin{tabular}{@{}l@{}} 
      Mitigate  
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      \textit{Can we mitigate biases?}
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Feature selection
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Fair algorithm (ACF)
      \end{tabular} &
      \begin{tabular}{@{}l@{}} 
      Reranking for fair \\
      allocation (FA*IR)
      \end{tabular} &
      
      \bottomrule
    \end{tabular}
    \end{center}
\end{table*}

\section{Method}
\label{sec:method}
\name provides the full support of the proposed framework in Section \ref{sec:framework} in the system. In this section, we explain how we implement the fair decision making framework with our perspectives, measures, and methods described in Table \ref{tbl:framework}. We also elaborate on how they are related to the specific context of ranking decision.

\subsection{Understanding Bias}
\label{sec:method_understanding_bias}
\name accommodates the intuitive understanding of machine learning task with the perspective of space. To be specific, we define \data and \outcome phases as two spaces (\inputspace and \outputspace Space), and the machine learning process as \textit{"the interactions between different spaces that make up the decision pipeline for a task"}, inspired by \cite{friedler2016possibility} (Fig. \ref{fig:teaser}a). Input space is a metric space of Data stage where individuals represented as a set of features reside in. When we process data with a machine learning model, it is mapping individuals from Input space to Output space. In this setting, bias can be introduced in each space or within the interaction of two spaces. Our visual analytic tool visualizes the distribution of individuals and groups in two spaces and the mapping, and provides the measures consistently defined with the perspective of space. 

{\bf Input space.} We define Input space $I(\mat{X}, I_\mat{X})$, where individuals are mapped to $p$-dimensional space with a set of $p$ number of feature values.

{\bf Mapping.} A machine learning model is a function $f:I -> O$ to map the individuals in the Input space $I$ to the Output space $O$.

{\bf Output space.} Output space $O$ is an ordered list where individuals are ranked by their qualifications. When a classification model is used, we calculate the probability of each individual being classified as positive, and assign them to discrete ranking.

\subsection{Measuring Bias} 
\label{sec:measuring_bias}
In our system, we implement \measure stage with multiple measures defined (Fig. \ref{fig:teaser}b). We take advantage of the perspective of space in Section \ref{sec:method_understanding_bias} that bias can be understood in three spaces, which is measurable and understandable. Given this perspective, we define the measure of different notion of fairness: Individual and Group fairness. In three spaces, bias is defined in a space or the mapping between spaces, then the fairness individuals and groups are measured in instance-level and global-level metrics to provide the comprehensive summary of bias. Along with fairness measures, we define the utility measures in the context of ranking decision. We start by discussing the definition of distance and distortion as the unit of measuring bias, then explain the details of fairness and utility measure in the following sections.

\subsubsection{Distance and Distortion in the space}
\label{sec:distance_distortion}
Distance and distortion are two basic notions in the system to measure bias. Given any two individuals $i, j$, a pairwise distance $d(i,j)$ indicates how two individuals are similar to each other in a space. When two individuals are mapped from one space to another, the pairwise distance may be preserved or not. We define distortion as the discrepancy between two pairwise distances, indicating that the mapping is not fair. In our system, we incorporate two pairwise distances for \inputspace and \outputspace space. For \inputspace space, we calculate the Gower distance \cite{gower1971general} between $\mat{X}'_i$ and $\mat{X}'_j$, which measures the pairwise distance of continuous and categorical variables separately and sum them up. For \outputspace space, the pairwise distance is simply the absolute ranking difference of two individuals $r_i, r_j$. Then we calculate the distortion of two spaces. Given two instances $i, j$, the distortion is the absolute difference of two normalized pairwise distances using min-max scaling from \inputspace space and \outputspace space. In our system, pairwise distortion is understood as a basic unit of mapping bias.
\begin{equation}
distortion_{(i,j)} = |d_I(\mat{X}'_i, \mat{X}'_j) - d_O(r_i, r_j)|
\end{equation}

\subsubsection{Individual Fairness}
\label{sec:individual_fairness}
Based on the definition of individual fairness, ``Similar individuals should be treated similarly'', \name defines Individual fairness as how the pairwise distances in \inputspace space are to be well-preserved in \outputspace space while mapping. Basically, this definition follows the definition of distortion between two pairwise distances in Section \ref{sec:distance_distortion}. The unit of Individual fairness is per-individual distortion as instance-level bias in the local level. When we sum up all instance-level bias, we can obtain the global individual fairness. \name provides both levels of Individual fairness to support different levels of  exploration.

\textbf{Instance-level bias.} Instance-level measure is the amount of distortion with respect to an individual from the pairwise distance to other similar individuals. We define the realization of "similar individuals" of an individual $n_l$ as its 4 nearest neighbors (h=4) noted by $NN_h$. Here, nearest neighbors are individuals that have the most similar qualification (i.g., the closest neighbors in the Input space) in \inputspace space. Then we measure how an individual and its nearest neighbors in \inputspace space are close to each other in the ranking outcome. We subtract 1 by the distance to notate the similarity. The measure closer to 1.0 indicates that the instance is more fairly treated compared to its neighbors. 

\begin{equation} \label{eq:rnn}
rNN_l=1-\frac{1}{h} \sum_{l\in N, m \in NN_h(n_l)} \frac{|r_l - r_m|}{|C|}
\end{equation}


While $rNN$ quantifies the amount of bias with respect to an individual, bias may be disadvantaged  (i.g., ranked higher than its neighbors), or advantaged to an individual (i.g., ranked lower than its neighbors). We see that it is also important to reveal whether the distortion had been beneficial or detrimental as the consequence of bias. For this purpose, rNN-gain is to quantify the signed ranking distortion in order to reveal the ranking gain. \\
\begin{equation}
rNN_{gain}=1-\frac{1}{h} \sum_{l\in N, m \in NN_h(n_l)} \frac{(r_l - r_m)}{|C|}
\end{equation}

\textbf{Global-level bias.} Individual fairness as a global measure of all individuals is measured by averaging all instance-level biases to indicate how greatly individuals were biased compared to their similar individuals in overall.

\begin{equation}
rNN_{mean}= \frac{1}{n} \sum_{l\in k} rNN_l
\end{equation}

\subsubsection{Group Fairness}
\label{sec:group_fairness}
While Individual fairness treats each individual  independently, Group fairness treats an individual as a member of a group. With a protected and non-protected group defined in our system, Group fairness measures whether two groups are fairly distributed within a specific space (\inputspace and \outputspace bias). For \mappingspace space, any pair of individuals are also treated as within-group pair (i,g, a pair of individuals from the same group) or between-group pair (i,g, a pair of individuals from different groups), whose distortions are calculated to measure the mapping bias. \\

{\bf Data bias.} Data bias for Group fairness is to measure whether there have been biases already inherent in the dataset. In the framework, \inputspace space consists of individuals in $p$-dimensional feature space defined by $p$ number of features selected. When we treat two groups as a set of points in a metric space, Group fairness in \inputspace space is defined as the degree of separation of two groups (i.g., two clusters). We name it Group Separateion score. We adopt Hausdorff distance \cite{hausdorff2005set} to measure the separation of two sets of individuals. Here, we incorporate Gower distance as the pairwise distance $d(a, b)$. The one-sided Hausdorff distance from A to B is defined as:

\begin{equation}
\tilde{h}(A,B)=max_{a \in A} \{min_{b \in B}~d(a,b) \}
\end{equation}

and then the bidirectional Hausdorff distance between A and B is:

\begin{equation}
h(A,B)=max( \tilde{h}(A,B), \tilde{h}(B,A))
\end{equation}

{\bf Mapping bias.} In \mappingspace space, any pair of two individuals $i, j$ as membership of two groups is defined as one of two kinds of pairs: between-group (i.g., $i \in S^+,~j \in S^-$) and within-group pairs (i.g., $i,j \in S^{(\cdot)}$). Mapping bias in Group fairness also measures the distortion in the pairwise distances of \inputspace and \outputspace space as mentioned in Section \ref{sec:distance_distortion} but calculates it in terms of group fairness. Our concern is to measure how great between-group distortion is. For examples, when the pairwise distances between Men and Women (between-group distortion) are greater, the structure of two groups in \inputspace Space will not be preserved while mapping by unequal treatment. We adopt Group Skew measure proposed by \cite{friedler2016possibility}, to measure the relative greatness of between-group distortion over within-group distortion. When between-group distortion is greater than within-group distortion (Group Skew $>$ 1), we call it Structural bias as defined by \cite{friedler2016possibility}. \\
\begin{equation}
\begin{aligned}
& Group~Skew = \frac{Distortion_{BTN}}{Distortion_{WTN}} \\
& where \\
& Distortion_{BTN}=\sum_{i \in S^+, j \in S^-,i \ne j}distortion(i,j) \\
& Distortion_{WTN}=\sum_{i,j \in S^{(\cdot)},i \ne j}distortion(i,j)
\end{aligned}
\end{equation}

{\bf Mapping bias in group.} We also measure how each group as a set of individuals obtains the mapping bias. Based on Equation \ref{eq:rnn}, the group-level bias is calculated by averaging all biases of individuals that belong to the protected group $S^+$ or non-protected group $S^-$:

\begin{equation}
\begin{aligned}
& rNN_{S^+}= \frac{1}{|S^+|} \sum_{l \in S^+} rNN_l \\
& rNN_{S^-}= \frac{1}{|S^-|} \sum_{l \in S^-} rNN_l
\end{aligned}
\end{equation}

{\bf Context in Ranking Decision.}
Before we discuss about outcome bias, we give a brief background of the context of ranking decision, and define two types of ranking decision, between-ranking and within-ranking decision. First, we define between-ranking decision as the comparison between different rankings. Decision making in general is an iterative process until the decision maker finds an outcome that fits best in their goal. In the context of ranking decision, decision makers iterate over the process multiple times, compare multiple rankings, and find the best ranking $R_k$ among generated rankings. We refer to this type of decision as between-ranking decision since this is a decision making between ranking. Separate from between-ranking decision, we define within-ranking decision, as another type of ranking decision to decide how many individuals they are going to pick with the \topk threshold within a specific ranking. In other words, within-ranking decision is to compare the condition with different thresholds (e.g., $R_k$ vs. $R_{k+1}$) with respect to a ranking outcome. We incorporate these two types of  ranking decisions for both fairness and utility.

\name defines the measures of between-ranking and within-ranking decision to consider their different contexts of decision making. For the between-ranking measure, we start from the widely used ranking metrics such as nDCG. It involves ranking discount for between-ranking decision so that rankings with the same item set but are ordered differently have different scores. Such ranking metrics take the logarithmic discount to favor items within the top ranking to reflect the nature of information retrieval or recommendation system where exposures and attentions of users are skewed towards a few items. On the other hand, we claim that ranking in decision making is in a different situation where the individuals within the \topk list are not judged by attentions or scores but treated equally once they get in the list. From the observation, we adjust a lenient discount, which is linearly proportional to the number of whole instances n, to differentiate the rankings with different orders but in a way that it does not significantly favors the top items.

For within-ranking decision, it is the matter of setting up the \topk threshold where we compare two rankings $R_{i=1,...,k}$ and $R_{i=1,...,k+m}$. In other words, it compares a ranking instance $R_k$ with top $k$ threshold, with the same ranking instance $R_{k+\alpha}$ with threshold $k+\alpha$. Here, the discount of ranking is not applied to the local measure such that the difference of two ranking representations coming from instances ${k+1, k+2, ..., k+\alpha}$ is not collapsed by the greater influence of top ranking instances with ranking discount.

{\bf Outcome bias.} Given the context in ranking decision as discussed in the previous section, we define the between-ranking and within-ranking measure separately. 
\edit{We propose GFDCG} as the between-ranking fairness measure with multiple criteria, which compares two groups by the proportion of the quality of \topk ranked individuals. It counts whether each individual deserves a positive outcome by looking at target value $\hat{y}$ with linear ranking discount. On the other hand, the within-ranking fairness measure is the statistical parity of two groups to solely focus on comparing the group ratios within top k threshold. \\
\begin{equation}
\begin{aligned}
 & GFDCG@k=\frac{linear~DCG@k(S^+)}{linear~DCG@k(S^-)} \\
 & where~linear~DCG@k(S^{(\cdot)}) = \sum_{i \in S^{(\cdot)} \cap N^{topk}} y_i \times \frac{n-r_i}{n}
\end{aligned}
\end{equation}

\subsubsection{Utility} We define the utility of a ranking as the qualification of individuals. It ultimately indicates how selected individuals within \topk threshold are qualified. Utility also shares the context of two ranking decisions: Within-ranking and between-ranking utility. Between-ranking utility follows the original nDCG measure \cite{jarvelin2002cumulated} but we apply  linear ranking discount instead of logarithmic discount. For Ideal DCG (IDCG), individuals are ordered by their target values, noted by $N_{I}$, where individuals with positive target labels are ranked higher:

\begin{equation}
\begin{aligned}
 & linear~nDCG@k = \frac{linear~DCG@k}{linear~IDCG@k} \\
 & where \\
 & linear~DCG@k = \frac{}{}\sum_{i \in N^{topk}} y_i \times \frac{n-r_i}{n} \\
 & linear~IDCG@k = \frac{}{}\sum_{i \in N_{I}^{topk}} y_i \times \frac{n-r_i}{n}
\end{aligned}
\end{equation}

On the other hand, with-ranking measure is simply following Precision@k which sums up all the true labels without ranking discount to compare the different \topk threshold for a specific ranking. 

\subsection{Identifying Bias} 
\label{sec:identify_bias}
The system provides three ways of detecting the possibility of features bringing in biases for each machine learning phase: (1) \data: Feature correlation between sensitive attribute and each feature, (2) \model: Per-feature difference between outliers of distortion and whole instances, and (3) \outcome: Feature importance by ranking perturbation.

{\bf Feature correlation.} In \data phase, we support the feature correlation analysis to capture bias within each feature for Group fairness. Recall that the goal of Group fairness in \inputspace space is to remove the information that can indicate the membership of individuals. In this context, any features other than the sensitive attribute may include the information such that it correlates to the sensitive attribute (e.g., height of men and women). We detect the correlation between the sensitive attribute and each feature by comparing the two group distribution of each feature value. If two distributions for protected group and non-protected group of a feature $\vec{x}_p$ are very distinct from each other, such features are likely to be used as a proxy variable of the sensitive attribute. 

We calculate Wasserstein distance of two distributions to measure the possibility of each feature being a proxy variable and provide the distance as correlation between each feature and the sensitive attribute. It calculates the transportation cost to move from one distribution to another. Wasserstein distance \cite{ruschendorf2001wasserstein} fits our setting in that it can not only handle both continuous and categorical distributions, but also is a symmetric measure with allowing the possibility of zero entry. Given a feature $\vec{x}_p$, $W(S^+_{x_i}, S^-_{x_j})$ calculates how greater the distributions of two groups are. The greater the distance, the two groups are distinguishable by leveraging the feature, which leads to indirect discrimination. 

{\bf Feature distortion by outliers.} In \model phase, we analyze how each feature is correlated to the overall distortions. We first draw the overall distribution plot of instances' distortion in the mapping. Then we identify the outliers that have greater distortions than others (i.g., top 5\% in the distribution of distortions). We compare the distribution of outliers vs. all other individuals with respect to each feature value. It ultimately reveals which feature is correlated to the outliers. We compute the Wasserstein distance between the distribution of outliers and whole individuals, and provide the scores for each feature.

{\bf Feature perturbation.} In \outcome phase, we analyze the importance of each feature with respect to the quality of ranking outcome. Here, we take the feature perturbation method \cite{breiman2001random}, a well-known auditing technique to experiment how each feature contributes to utility and fairness. First, we permute the values of a feature $\vec{x}_q$ from $\mat{X}'$ and retrain the model with $\mat{X}'={\vec{x}_1, ...,\vec{x}_p, \vec{x}_q}$. Then we measure its importance by how great the measures drop compared to the original performance. In the ranking decision within our system, we permute the values of a feature $\vec{x}_q$ by swapping a feature values of $\vec{x}_{i1}, \vec{x}_{i2}, ..., \vec{x}_{i(2/n)}$ with $\vec{x}_{i(2/n+1)}, ..., \vec{x}_{in}$ as proposed by \cite{fisher2018model}, and retrain the model. We calculate the drop rate of utility and fairness. If a feature has a severe drop rate, it contributes to more accurate and fair outcome. If a feature has decreasing fairness, on the other hand, they are likely to be a potential source of bias.


\subsection{Mitigating bias} \label{mitigating_bias}
FairSight supports a complete package of reducing biases in three phases of the machine learning pipeline. In this section, we explain the details of pre-processing, in-processing, and post-processing method.

{\bf Pre-precessing.} Pre-processing is a preemptive action to obtain a set of features $X'$ that are as less biased as possible. To achieve Group fairness, the first step is to exclude the sensitive attribute in representing individuals. This is to explicitly declare that we do not consider the sensitive attribute in the decision making. As mentioned in Section \ref{sec:identify_bias}, any other features may correlate to the sensitive attribute so that they bring in indirect discrimination. Any features detected in \identify stage can be excluded in the selected feature $X'$.

{\bf In-precessing.} In-processing method is to mitigate bias with the selection of fair algorithms. \name adopts Additive Counterfactually Fair (ACF) model proposed by \cite{kusner2017counterfactual}. The method is based on the assumption that for each individual, two counterfactual probabilities where the individual belongs to either protected group or non-protected group should be the same regarding a feature. A variety of fair algorithms as in-processing methods are likely to be plugged in the system as additional modules based on users' needs.

{\bf Post-precessing.} Post-processing method is to achieve the fair ranking outcome independently of \data and \model phase. Given a ranking outcome $R$, a post-processing method mitigates bias by manipulating the ranking.
This module especially fits into some situations where decision makers are not able to fully control over every step of the machin learning task. When they have access just to the ranking outcome without modifying data and model, the post-processing method serves as only strategy to mitigate bias. In our system, we introduce a fair algorithm proposed by \cite{zehlike2017fa}. It re-ranks a ranking outcome by randomly picking an individual from the ranking of two groups with the assigned probabilities. 

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

